Flavor changing neutral decay effects in models with two Higgs boson doublets: Applications to LHC Physics

In this Thesis we have investigated some effects appearing in top quark and Higgs boson decays with flavor changing neutral currents (FCNC) in the framework of generic Two Higgs Doblet Models (2HDM) and the Minimal Supersymmetric Standard Model (MSSM). We have applied these two extensions to the SM to see whether they can produce new FCNC effects. Introductory chapters deal with the 2HDM and the MSSM. In the next chapters we have computed the following FCNC decays: (1) the branching ratios (B) of the top quark to Higgs bosons and charm quark in the 2HDM; (2) B and number of events at the Large Hadron Collider (LHC) of the Higgs bosons to top and charm quarks in the 2HDM; (3) B of the Higgs bosons to bottom and strange quarks in the MSSM; (4) cross section and number of events at the LHC of the Higgs bosons to FCNC final states involving the heavy quarks like the top and bottom quark in the MSSM (Higgs bosons = h^0, H^0, A^0). We also studied the experimental signatures that would allow discover of the nature of these Higgs bosons in the LHC. In this study we have applied the severe restrictions from observed low-energy FCNC processes like b -> s\gamma. Our general conclusion is that the physics of the processes with flavor changing neutral currents can be very important in seeing the physics beyond the Standard Model and to disentangle the nature of the most adequate model. Experiments at the LHC can be crucial to unravel signs of FCNC physics beyond the SM.

==> hbsSUSY_prod/Makefile <==
# $Id: /susy/mirror/trunk/article_prod/Makefile 699 2005-08-01T08:46:50.868654Z guasch  $

AGR = $(wildcard *.agr)
EPS = $(AGR:.agr=.eps)

PW=$(shell basename $(PWD))
VER=$(shell svnversion -n . | tr \: _)


all: eps

eps: $(EPS)

%.eps: %.agr
	LC_ALL=C gracebat -hdevice EPS -printfile $@ $<

ps: article.ps

pdf: article.pdf

article.ps: article.dvi $(EPS)
	dvips -o $@ $<

article.pdf: article.ps
	ps2pdf article.ps 

article.dvi: article.tex $(EPS) 
	latex $<

bib: article.bbl

article.bbl: hbssqcd.bib article.dvi
	bibtex article

tar: article-$(VER).tar.gz 

article-$(VER).tar.gz:  article.ps history.txt
	mkdir -p article-$(VER)
	cp -a $(EPS) article.ps *tex *sty *bib *bbl *bst history.txt article-$(VER)
	tar -zcvf article-$(VER).tar.gz article-$(VER)
	rm -rf article-$(VER)

history.txt: $(AGR) article.tex Makefile hbssqcd.bib
	svn log -v > history.txt

article: eps 
	latex article
	$(MAKE) bib
	latex article
	latex article 
	latex article
	$(MAKE) ps 

everything: article  tar

clean:
	rm -f $(EPS)
# $Id: /susy/mirror/trunk/article_prod/Makefile 699 2005-08-01T08:46:50.868654Z guasch  $

